Numerical Study of the Spin-1 Antiferromagnetic Heisenberg Chain with a Spin-1/2 Impurity

Low-lying excited states as well as the ground state of the spin-1 antiferromagnetic Heisenberg chain with a spin-1/2 impurity are studied by means of a method of numerical diagonalization. The isotropic nearest-neighbor exchange coupling plus the uniaxial single-ion-type anisotropy energy is assumed for the host-system Hamiltonian. The energy differences between the ground state and the low-lying excited states, which appear in the Haldane gap, are estimated in the thermodynamic limit. The results are used to analyze the electron-spin-resonance experimental data on Ni(C$_2$H$_8$N$_2$)$_2$NO$_2$(ClO$_4$), abbreviated NENP, containing a small amount of spin-1/2 Cu$^{2+}$ impurities. It is found that in this system, the impurity-host $\bigl($Cu$^{2+}$-Ni$^{2+}$$\bigr)$ coupling is ferromagnetic and its magnitude is about 5$\,$\% of the magnitude of the host-host $\bigl($Ni$^{2+}$-Ni$^{2+}$$\bigr)$ coupling.

==> table1.tex <==
%
%1995-02-15
%TMT1.TEX
%

\magnification=\magstep1
\hsize=24.7truecm
\vsize=17.4truecm
\hoffset=-0.15truein
\voffset=-0.22truein

\baselineskip=15.0pt

\nopagenumbers

{\leftskip=1.5pc
\parindent=-1.5pc
Table~\uppercase\expandafter{\romannumeral1}$\,$.$\ \ $Finite-$N$ values of
$\epsilon_{(1/2,+)}(N)/J$, $\epsilon_{(1/2,-)}(N)/J$,
$\epsilon_{(1/2,+)'}(N)/J$, and $\epsilon_{(3/2,+)}(N)/J$ for $d\!=\!0.0$,
calculated for various values of $J'/J$.  Note that
$\epsilon_{(1/2,+)'}(N)\!=\!\epsilon_{(3/2,+)}(N)$ when $J'\!>\!0$ and
$\epsilon_{(3/2,+)}(N)\!=\!\epsilon_{(1/2,+)}(N)$ when $J'\!<\!0$. \par}

\vskip 10.0pt

{\leftskip=1.5pc
\parindent=+0.3pc
(a)~~$\epsilon_{(1/2,+)}(N)/J$ \par}

\vskip -10pt

$$\vbox{
\halign{\hfil#      &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil                                \cr
%
\multispan8\hrulefill\cr
%
$J'/J $ & $N\!=\! 5$   & $N\!=\! 7$   & $N\!=\! 9$   & $N\!=\!11$
        & $N\!=\!13$   & $N\!=\!15$   & $N\!=\!17$                     \cr
%
\multispan8\hrulefill\cr
%
$-0.30$ & $ -6.054182$ & $ -8.848086$ & $-11.640230$ & $-14.433542$
        & $-17.228587$ & $-20.025297$ & $-22.823434$                   \cr
%
$-0.20$ & $ -5.974922$ & $ -8.771783$ & $-11.565739$ & $-14.360276$
        & $-17.156197$ & $-19.953554$ & $-22.752176$                   \cr
%
$-0.10$ & $ -5.899732$ & $ -8.699949$ & $-11.495923$ & $-14.291798$
        & $-17.088660$ & $-19.886704$ & $-22.685835$                   \cr
%
$ 0.00$ & $ -5.830213$ & $ -8.634532$ & $-11.432932$ & $-14.230359$
        & $-17.028266$ & $-19.827036$ & $-22.626684$                   \cr
%
$ 0.10$ & $ -5.963368$ & $ -8.759273$ & $-11.552826$ & $-14.347250$
        & $-17.143216$ & $-19.940695$ & $-22.739468$                   \cr
%
$ 0.20$ & $ -6.098600$ & $ -8.887590$ & $-11.677328$ & $-14.469455$
        & $-17.263959$ & $-20.060471$ & $-22.858588$                   \cr
%
$ 0.30$ & $ -6.235457$ & $ -9.018623$ & $-11.805252$ & $-14.595543$
        & $-17.388888$ & $-20.184637$ & $-22.982234$                   \cr
%
\multispan8\hrulefill\cr
%
}}$$

\vskip 10.0pt

{\leftskip=1.5pc
\parindent=+0.3pc
(b)~~$\epsilon_{(1/2,-)}(N)/J$ \par}

\vskip -10pt

$$\vbox{
\halign{\hfil#      &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil                                \cr
%
\multispan8\hrulefill\cr
%
$J'/J $ & $N\!=\! 5$   & $N\!=\! 7$   & $N\!=\! 9$   & $N\!=\!11$
        & $N\!=\!13$   & $N\!=\!15$   & $N\!=\!17$                     \cr
%
\multispan8\hrulefill\cr
%
$-0.30$ & $ -5.309153$ & $ -8.328417$ & $-11.246685$ & $-14.117088$
        & $-16.962018$ & $-19.792251$ & $-22.613495$                   \cr
%
$-0.20$ & $ -5.295485$ & $ -8.315081$ & $-11.232456$ & $-14.101753$
        & $-16.945633$ & $-19.774940$ & $-22.595395$                   \cr
%
$-0.10$ & $ -5.286686$ & $ -8.306572$ & $-11.223408$ & $-14.092010$
        & $-16.935219$ & $-19.763931$ & $-22.583876$                   \cr
%
$ 0.00$ & $ -5.283567$ & $ -8.303576$ & $-11.220229$ & $-14.088587$
        & $-16.931557$ & $-19.760055$ & $-22.579814$                   \cr
%
$ 0.10$ & $ -5.286954$ & $ -8.306811$ & $-11.223658$ & $-14.092287$
        & $-16.935527$ & $-19.764271$ & $-22.584247$                   \cr
%
$ 0.20$ & $ -5.297593$ & $ -8.316962$ & $-11.234436$ & $-14.103943$
        & $-16.948071$ & $-19.777637$ & $-22.598345$                   \cr
%
$ 0.30$ & $ -5.316038$ & $ -8.334613$ & $-11.253235$ & $-14.124347$
        & $-16.970116$ & $-19.801221$ & $-22.623324$                   \cr
%
\multispan8\hrulefill\cr
%
}}$$

\vfill\eject

{\leftskip=1.5pc
\parindent=+0.3pc
(c)~~$\epsilon_{(1/2,+)'}(N)/J$ \par}

\vskip -10pt

$$\vbox{
\halign{\hfil#      &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil                                \cr
%
\multispan8\hrulefill\cr
%
$J'/J $ & $N\!=\! 5$   & $N\!=\! 7$   & $N\!=\! 9$   & $N\!=\!11$
        & $N\!=\!13$   & $N\!=\!15$   & $N\!=\!17$                     \cr
%
\multispan8\hrulefill\cr
%
$-0.30$ & $ -5.451354$ & $ -8.298314$ & $-11.125222$ & $-13.942842$
        & $-16.755529$ & $-19.565325$ & $-22.373296$                   \cr
%
$-0.20$ & $ -5.573010$ & $ -8.401564$ & $-11.215359$ & $-14.023132$
        & $-16.828188$ & $-19.631956$ & $-22.435105$                   \cr
%
$-0.10$ & $ -5.699777$ & $ -8.514645$ & $-11.319475$ & $-14.121061$
        & $-16.921741$ & $-19.722387$ & $-22.523314$                   \cr
%
$ 0.00$ & $ -5.830213$ & $ -8.634532$ & $-11.432932$ & $-14.230359$
        & $-17.028266$ & $-19.827036$ & $-22.626684$                   \cr
%
\multispan8\hrulefill\cr
%
}}$$

\vskip 10.0pt

{\leftskip=1.5pc
\parindent=+0.3pc
(d)~~$\epsilon_{(3/2,+)}(N)/J$ \par}

\vskip -10pt

$$\vbox{
\halign{\hfil#      &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil                                \cr
%
\multispan8\hrulefill\cr
%
$J'/J $ & $N\!=\! 5$   & $N\!=\! 7$   & $N\!=\! 9$   & $N\!=\!11$
        & $N\!=\!13$   & $N\!=\!15$   & $N\!=\!17$                     \cr
%
\multispan8\hrulefill\cr
%
$ 0.00$ & $ -5.830213$ & $ -8.634532$ & $-11.432932$ & $-14.230359$
        & $-17.028266$ & $-19.827036$ & $-22.626684$                   \cr
%
$ 0.10$ & $ -5.768795$ & $ -8.578704$ & $-11.380467$ & $-14.180017$
        & $-16.979284$ & $-19.778923$ & $-22.579116$                   \cr
%
$ 0.20$ & $ -5.719142$ & $ -8.537588$ & $-11.344937$ & $-14.148268$
        & $-16.950089$ & $-19.751407$ & $-22.552650$                   \cr
%
$ 0.30$ & $ -5.686463$ & $ -8.518738$ & $-11.336204$ & $-14.147241$
        & $-16.955021$ & $-19.760967$ & $-22.565797$                   \cr
%
\multispan8\hrulefill\cr
%
}}$$

\bye


==> table2.tex <==
%
%1995-03-06
%TMT2.TEX
%

\magnification=\magstep1
\hsize=6.46truein
\vsize=8.89truein
\hoffset=-0.25truein
\voffset=0.01truein

\baselineskip=15.0pt

\nopagenumbers

{\leftskip=1.5pc
\parindent=-1.5pc
Table~\uppercase\expandafter{\romannumeral2}$\,$.$\ \ $Estimated values of
${\tilde\Delta}_{(1/2,-)}$, ${\tilde\Delta}_{(1/2,+)'}$, and
${\tilde\Delta}_{(3/2,+)}$ for $d\!=\!0.0$ and $d\!=\!0.2$.  Note
that ${\tilde\Delta}_{(3/2,+)}\!=\!{\tilde\Delta}_{(1/2,+)'}$ when $d\!=\!0.0$.
\par}

\vskip 10.0pt

$$\vbox{
\halign{\hfil#      &\qquad \hfil#      &\qquad \hfil#      &\qquad
        \hfil#      &\qquad \hfil#      &\qquad \hfil#                     \cr
%
\multispan6\hrulefill\cr
%
              & $d\!=\!0.0\qquad\qquad$\span\omit
              & $d\!=\!0.2\qquad\qquad\qquad\quad$\span\omit\span\omit          \cr
%
 $\ J'/J\;$ & \multispan5\hrulefill\cr
%
              & ${\tilde\Delta}_{(1/2,-)}$ & ${\tilde\Delta}_{(1/2,+)'}$
              & ${\tilde\Delta}_{(1/2,-)}$ & ${\tilde\Delta}_{(1/2,+)'}$
              & ${\tilde\Delta}_{(3/2,+)}$                                 \cr
%
\multispan6\hrulefill\cr
%
 $-0.20$ & $-0.2015$ & $-0.3045$ & $-0.1728$ & $-0.2929$ & $-0.2609$       \cr
 $-0.15$ & $-0.1560$ & $-0.2337$ & $-0.1379$ & $-0.2307$ & $-0.2056$       \cr
 $-0.10$ & $-0.1061$ & $-0.1580$ & $-0.0944$ & $-0.1585$ & $-0.1409$       \cr
 $-0.08$ & $-0.0855$ & $-0.1269$ & $-0.0756$ & $-0.1277$ & $-0.1134$       \cr
 $-0.06$ & $-0.0646$ & $-0.0954$ & $-0.0561$ & $-0.0957$ & $-0.0852$       \cr
 $-0.04$ & $-0.0435$ & $-0.0637$ & $-0.0361$ & $-0.0623$ &                 \cr
 $-0.02$ & $-0.0223$ & $-0.0319$ &           &           &                 \cr
 $ 0.02$ & $ 0.0202$ & $ 0.0319$ &           &           &                 \cr
 $ 0.03$ &             &         & $ 0.0309$ &           &                 \cr
 $ 0.04$ & $ 0.0415$ & $ 0.0636$ & $ 0.0434$ & $ 0.0607$ & $ 0.0549$       \cr
 $ 0.06$ & $ 0.0626$ & $ 0.0952$ & $ 0.0659$ & $ 0.0953$ & $ 0.0836$       \cr
 $ 0.08$ & $ 0.0836$ & $ 0.1265$ & $ 0.0869$ & $ 0.1290$ & $ 0.1106$       \cr
 $ 0.10$ & $ 0.1044$ & $ 0.1573$ & $ 0.1072$ & $ 0.1623$ & $ 0.1365$       \cr
 $ 0.15$ & $ 0.1555$ & $ 0.2314$ & $ 0.1565$ & $ 0.2434$ & $ 0.1959$       \cr
 $ 0.20$ & $ 0.2048$ & $ 0.2990$ & $ 0.2036$ & $ 0.3179$ & $ 0.2444$       \cr
%
\multispan6\hrulefill\cr
%
}}$$

\bye


==> table3.tex <==
%
%1995-03-16
%TMT3.TEX
%

\magnification=\magstep1
\hsize=6.46truein
\vsize=8.89truein
\hoffset=-0.25truein
\voffset=0.01truein

\baselineskip=15.0pt

\nopagenumbers

{\leftskip=1.5pc
\parindent=-1.5pc
Table~\uppercase\expandafter{\romannumeral3}$\,$.$\ \ $Estimated values of
the coefficients $a_{(M,P)}$ and $b_{(M,P)}$. \par}

\vskip 10.0pt

$$\vbox{
\halign{\hfil#\hfil &\quad\qquad \hfil#\hfil &\quad \hfil#\hfil
                    &\quad\qquad \hfil#\hfil &\quad \hfil#\hfil
                    &\quad\qquad \hfil#\hfil &\quad \hfil#\hfil           \cr
%
\multispan7\hrulefill\cr
%
$d$ & $a_{(1/2,-)}$   & $b_{(1/2,-)}$
    & $a_{(1/2,+)'}$  & $b_{(1/2,+)'}$
    & $a_{(3/2,+)}$   & $b_{(3/2,+)}$                                     \cr
%
\multispan7\hrulefill\cr
%
 $ 0.0$ & $1.065$ & $0.018$ & $1.599$ & $   -0.063$ & $1.599$ & $-0.063$  \cr
 $ 0.1$ & $1.036$ & $0.217$ & $1.604$ & $\ \ 0.163$ & $1.539$ & $-0.290$  \cr
 $ 0.2$ & $1.026$ & $0.418$ & $1.618$ & $\ \ 0.293$ & $1.426$ & $-0.210$  \cr
 $ 0.3$ & $1.014$ & $0.470$ & $1.628$ & $\ \ 0.361$ & $1.325$ & $-0.117$  \cr
 $ 0.4$ & $0.990$ & $0.436$ & $1.627$ & $\ \ 0.467$ & $1.230$ & $-0.022$  \cr
%
\multispan7\hrulefill\cr
%
}}$$

\bye


==> table4.tex <==
%
%1995-02-18
%TMT4.TEX
%

\magnification=\magstep1
\hsize=24.7truecm
\vsize=17.4truecm
\hoffset=-0.15truein
\voffset=-0.22truein

\baselineskip=15.0pt

\nopagenumbers

{\leftskip=1.5pc
\parindent=-1.5pc
Table~\uppercase\expandafter{\romannumeral4}$\,$.$\ \ $Finite-$N$ values of
$\epsilon_{(1/2,+)}(N)/J$, $\epsilon_{(1/2,-)}(N)/J$,
$\epsilon_{(1/2,+)'}(N)/J$, and $\epsilon_{(3/2,+)}(N)/J$ for $d\!=\!0.2$,
calculated for various values of $J'/J$.

\vskip 10.0pt

{\leftskip=1.5pc
\parindent=+0.3pc
(a)~~$\epsilon_{(1/2,+)}(N)/J$ \par}

\vskip -3pt

$$\vbox{
\halign{\hfil#      &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil                                \cr
%
\multispan8\hrulefill\cr
%
$J'/J $ & $N\!=\! 5$   & $N\!=\! 7$   & $N\!=\! 9$   & $N\!=\!11$
        & $N\!=\!13$   & $N\!=\!15$   & $N\!=\!17$                     \cr
%
\multispan8\hrulefill\cr
%
$-0.30$ & $ -5.475582$ & $ -8.012057$ & $-10.546742$ & $-13.082394$
        & $-15.619570$ & $-18.158260$ & $-20.698299$                   \cr
%
$-0.20$ & $ -5.394812$ & $ -7.933029$ & $-10.468686$ & $-13.004973$
        & $-15.542612$ & $-18.081661$ & $-20.621989$                   \cr
%
$-0.10$ & $ -5.320835$ & $ -7.860148$ & $-10.396151$ & $-12.932553$
        & $-15.470260$ & $-18.009387$ & $-20.549817$                   \cr
%
$ 0.00$ & $ -5.275712$ & $ -7.814208$ & $-10.348532$ & $-12.882930$
        & $-15.418570$ & $-17.955715$ & $-20.494320$                   \cr
%
$ 0.10$ & $ -5.346869$ & $ -7.886106$ & $-10.423171$ & $-12.961113$
        & $-15.500510$ & $-18.041297$ & $-20.583261$                   \cr
%
$ 0.20$ & $ -5.471736$ & $ -8.006562$ & $-10.541781$ & $-13.078873$
        & $-15.617811$ & $-18.158295$ & $-20.700019$                   \cr
%
$ 0.30$ & $ -5.604929$ & $ -8.134761$ & $-10.667516$ & $-13.203229$
        & $-15.741312$ & $-18.281218$ & $-20.822527$                   \cr
%
\multispan8\hrulefill\cr
%
}}$$

\vskip 10.0pt

{\leftskip=1.5pc
\parindent=+0.3pc
(b)~~$\epsilon_{(1/2,-)}(N)/J$ \par}

\vskip -3pt

$$\vbox{
\halign{\hfil#      &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil                                \cr
%
\multispan8\hrulefill\cr
%
$J'/J $ & $N\!=\! 5$   & $N\!=\! 7$   & $N\!=\! 9$   & $N\!=\!11$
        & $N\!=\!13$   & $N\!=\!15$   & $N\!=\!17$                     \cr
%
\multispan8\hrulefill\cr
%
$-0.30$ & $ -4.652876$ & $ -7.417147$ & $-10.081405$ & $-12.698384$
        & $-15.290182$ & $-17.867362$ & $-20.435485$                   \cr
%
$-0.20$ & $ -4.639113$ & $ -7.403702$ & $-10.067030$ & $-12.682847$
        & $-15.273516$ & $-17.849668$ & $-20.416878$                   \cr
%
$-0.10$ & $ -4.630245$ & $ -7.395117$ & $-10.057884$ & $-12.672970$
        & $-15.262916$ & $-17.838405$ & $-20.405022$                   \cr
%
$ 0.00$ & $ -4.627100$ & $ -7.392093$ & $-10.054669$ & $-12.669498$
        & $-15.259185$ & $-17.834435$ & $-20.400836$                   \cr
%
$ 0.10$ & $ -4.630519$ & $ -7.395361$ & $-10.058140$ & $-12.673254$
        & $-15.263234$ & $-17.838760$ & $-20.405414$                   \cr
%
$ 0.20$ & $ -4.641266$ & $ -7.405623$ & $-10.069054$ & $-12.685093$
        & $-15.276033$ & $-17.852479$ & $-20.419990$                   \cr
%
$ 0.30$ & $ -4.659906$ & $ -7.423472$ & $-10.088095$ & $-12.705821$
        & $-15.298533$ & $-17.876702$ & $-20.445846$                   \cr
%
\multispan8\hrulefill\cr
%
}}$$

\vfill\eject

{\leftskip=1.5pc
\parindent=+0.3pc
(c)~~$\epsilon_{(1/2,+)'}(N)/J$ \par}

\vskip -3pt

$$\vbox{
\halign{\hfil#      &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil                                \cr
%
\multispan8\hrulefill\cr
%
$J'/J $ & $N\!=\! 5$   & $N\!=\! 7$   & $N\!=\! 9$   & $N\!=\!11$
        & $N\!=\!13$   & $N\!=\!15$   & $N\!=\!17$                     \cr
%
\multispan8\hrulefill\cr
%
$-0.30$ & $ -4.813371$ & $ -7.412625$ & $\;\;-9.991555$ & $-12.560630$
        & $-15.124107$ & $-17.684056$ & $-20.241629$                   \cr
%
$-0.20$ & $ -4.931077$ & $ -7.511422$ & $-10.076178$ & $-12.633803$
        & $-15.187583$ & $-17.739067$ & $-20.289088$                   \cr
%
$-0.10$ & $ -5.050468$ & $ -7.617882$ & $-10.174052$ & $-12.725463$
        & $-15.274475$ & $-17.822158$ & $-20.369079$                   \cr
%
$ 0.00$ & $ -5.149004$ & $ -7.709056$ & $-10.261722$ & $-12.811685$
        & $-15.360390$ & $-17.908390$ & $-20.455944$                   \cr
%
$ 0.10$ & $ -5.139953$ & $ -7.693920$ & $-10.240734$ & $-12.785313$
        & $-15.329197$ & $-17.872962$ & $-20.416857$                   \cr
%
$ 0.20$ & $ -5.087907$ & $ -7.643786$ & $-10.191231$ & $-12.736204$
        & $-15.280593$ & $-17.825047$ & $-20.369784$                   \cr
%
$ 0.30$ & $ -5.042013$ & $ -7.604356$ & $-10.155913$ & $-12.704125$
        & $-15.251613$ & $-17.799457$ & $-20.348198$                   \cr
%
\multispan8\hrulefill\cr
%
}}$$

\vskip 10.0pt

{\leftskip=1.5pc
\parindent=+0.3pc
(d)~~$\epsilon_{(3/2,+)}(N)/J$ \par}

\vskip -3pt

$$\vbox{
\halign{\hfil#      &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil &\qquad \hfil#\hfil &\qquad
        \hfil#\hfil &\qquad \hfil#\hfil                                \cr
%
\multispan8\hrulefill\cr
%
$J'/J $ & $N\!=\! 5$   & $N\!=\! 7$   & $N\!=\! 9$   & $N\!=\!11$
        & $N\!=\!13$   & $N\!=\!15$   & $N\!=\!17$                     \cr
%
\multispan8\hrulefill\cr
%
$-0.30$ & $ -5.355288$ & $ -7.901662$ & $-10.446271$ & $-12.991136$
        & $-15.536428$ & $-18.082026$ & $-20.627815$                   \cr
%
$-0.20$ & $ -5.280562$ & $ -7.830554$ & $-10.377293$ & $-12.923541$
        & $-15.469803$ & $-18.016123$ & $-20.562476$                   \cr
%
$-0.10$ & $ -5.211118$ & $ -7.765469$ & $-10.314753$ & $-12.862610$
        & $-15.409957$ & $-17.957053$ & $-20.503988$                   \cr
%
$ 0.00$ & $ -5.149004$ & $ -7.709056$ & $-10.261722$ & $-12.811685$
        & $-15.360390$ & $-17.908390$ & $-20.455944$                   \cr
%
$ 0.10$ & $ -5.097223$ & $ -7.665435$ & $-10.223245$ & $-12.776551$
        & $-15.327447$ & $-17.876874$ & $-20.425345$                   \cr
%
$ 0.20$ & $ -5.059993$ & $ -7.640602$ & $-10.206973$ & $-12.766389$
        & $-15.321712$ & $-17.874371$ & $-20.425203$                   \cr
%
$ 0.30$ & $ -5.042625$ & $ -7.641730$ & $-10.221625$ & $-12.791271$
        & $-15.354531$ & $-17.913493$ & $-20.469438$                   \cr
%
\multispan8\hrulefill\cr
%
}}$$

\bye

